Fast Decentralized Linear Functions Over Edge Fluctuating Graphs

Implementing linear transformations is a key task in the decentralized signal processing framework, which performs learning tasks on data sets distributed over multi-node networks. That kind of network can be represented by a graph. Recently, some decentralized methods have been proposed to compute linear transformations by leveraging the notion of graph shift operator, which captures the local structure of the graph. However, existing approaches have some drawbacks such as considering some special instances of linear transformations, or reducing the family of transformations by assuming that a shift matrix is given such that a subset of its eigenvectors spans the subspace of interest. In contrast, this paper develops a framework for computing a wide class of linear transformations in a decentralized fashion by relying on the notion of graph shift operator. The main goal of the proposed method is to compute the desired linear transformation in a small number of iterations. To this end, a set of successive graph shift operators is employed, then, a new optimization problem is proposed whose goal is to compute the desired transformation as fast as possible. In addition, usually, the topology of the networks, especially the wireless sensor networks, change randomly because of node failures or random links. In this paper, the effect of edge fluctuations on the performance of the proposed method is studied. To deal with the negative effect of edge fluctuations, an online kernel-based method is proposed which enables nodes to estimate the missed values with their at hand information. The proposed method can also be employed to sparsify the network graph or reduce the number of local exchanges between nodes, which saves sensors power in the wireless sensor networks.

==> refs.tex <==


@inproceedings{barbarossa2009projection, 
	title={Distributed signal subspace projection algorithms with maximum convergence 	rate for sensor networks with topological constraints}, 
	author={S. Barbarossa and G. Scutari and T. Battisti}, 
	booktitle={International Conference on Acoustics, Speech, and Signal Processing (ICASSP)},
	month = {Apr.},
	year={2009},
	address={Taipei,Taiwan},
	pages={2893--2896}}

@inproceedings{romero2018projection, 
	title={Fast Decentralized Subspace Projection via Graph Filtering}, 
	author={T. Weerasinghe and  D. Romero and C. Asensio-Marco and B. Beferull-Lozano}, 
	booktitle={International Conference on Acoustics, Speech, and Signal Processing (ICASSP)}, 
	month = {Apr.},
	year={2018},
	address={Calgary,Canada},
	pages={4639--4643} 
}

@inproceedings{mollaebrahim2018projection, 
	title={DECENTRALIZED SUBSPACE PROJECTION IN LARGE NETWORKS}, 
	author={S. Mollaebrahim and   C. Asensio-Marco and D. Romero, and B. Beferull-Lozano}, 
	booktitle={Global Conference on Signal and Information Processing (GlobalSIP)}, 
	month = {Feb.},
	year={2018},
	address={Anaheim,USA},
	pages={788--792} 
}

@article{asensio2015energy, 
author={C. Asensio-Marco and B. Beferull-Lozano}, 
journal={IEEE Journal of Selected Topics in Signal Processing}, 
title={Energy Efficient Consensus Over Complex Networks}, 
year={2015}, 
volume={9}, 
number={2}, 
pages={292--303}, 
month={March}}

@article{chen2015ubiquitous, 
author={C. Chen and J. Yan and N. Lu and Y. Wang and X. Yang and X. Guan}, 
journal={IEEE Trans. on Emerging Topics in Comp.}, 
title={Ubiquitous Monitoring for Industrial Cyber-Physical Systems Over Relay- Assisted Wireless Sensor Networks}, 
year={2015}, 
volume={3}, 
number={3}, 
pages={352--362}, 
month={Sep.}}

@inproceedings{insausti2012projection, 
author={X. Insausti, P. M. Crespo and B. Beferull-Lozano}, 
booktitle={Int. Conf. on Dist. Comp. in Sensor Systems}, 
title={In-network Computation of the Transition Matrix for Distributed Subspace Projection}, 
year={2012}, 
volume={}, 
number={}, 
pages={124--131}, 
month={May}}



@article{segarra2017operators,
	title={Optimal Graph-Filter Design and Applications to Distributed Linear Network Operators},
	author={S. Segarra and A. G. Marques and A. Ribeiro},
	journal={IEEE Trans. Sig. Process.},
	volume={65},
	number={15},
	pages={4117--4131},
	month = {May},
	year={2017}
}
@article{segarra2017Network,
	title={Network topology inference from spectral templates},
	author={S. Segarra and A. G. Marques and G. Mateos and A. Ribeiro},
	journal={IEEE Trans. on Signal and Information Processing
over Networks,},
	volume={3},
	number={3},
	pages={467–483},
	month = {Sep},
	year={2017}
}

@inproceedings{sandryhaila2014finitetime, 
	title={Finite-time distributed consensus through graph filters}, 
	author={A. Sandryhaila and S. Kar and J. M. F. Moura}, 
	booktitle={International Conference on Acoustics, Speech, and Signal Processing (ICASSP)},
	month = {May},
	year={2014},
	address={Florence, Italy}, 
	pages={1080--1084}
}

@article{sandryhaila2013discrete, 
	title={Discrete signal processing on graphs:frequency analysis},
	author={A. Sandryhaila and J. M. F. Moura}, 
	journal={IEEE Trans. on Signal Processing}, 
	volume={61}, 
	number={7}, 
	pages={1644--1656}, 
	month = {Apr},
	year={2013}
}

@article{sandryhaila2014, 
	title={Discrete signal processing on graphs: Frequency Analysis},
	author={A. Sandryhaila and J. M. F. Moura}, 
	journal={IEEE Trans. on Signal Processing}, 
	volume={62}, 
	number={12}, 
	pages={3042--3054}, 
	month = {Jun},
	year={2014}
}
@article{chang2005projection, 
	title={Orthogonal subspace projection ({OSP}) revisited: a comprehensive study and analysis},
	author={Ch. Chang}, 
	journal={IEEE Trans. on Geoscience and Remote Sensing}, 
	volume={43}, 
	number={3}, 
	pages={502--518}, 
	month = {Mar.},
	year={2005}
}


@inproceedings{camaro2013reducing,
	title={Reducing the observation error in a WSN through a consensus-based subspace projection},
	author={F. Camaro-Nogues, D. Alonso-Roman, C. Asensio-Marco and B. Beferull-Lozano},
	booktitle={WCNC},
	month = {Apr.},
	year={2013},
	address={Shanghai,China},
	pages={3643--3648}
}

@book{bertsekas1999,
 	title={{N}onlinear {P}rogramming},
 	author={D. P. Bertsekas},
 	publisher={Athena scientific Belmont},
 	year={1999}
}

@Book{Golub,
	Title                    = {Matrix computations},
	Author                   = {Golub, G.H and Van Loan, C.F},
	Publisher                = {Johns Hopkins University Press},
	Year                     = {1996}
}
@Book{Horn,
	Title                    = {Matrix Analysis},
	Author                   = {Horn, R.A and Johnson, C.R},
	Publisher                = { Cambridge University Press},
	Year                     = {1995}
}

@Book{bishop,
	Title                    = {Pattern Recognition and Machine Learning},
	Author                   = { Bishop, C.M},
	Publisher                = {Springer},
	Year                     = {2006}
}

@Book{vetterli,
	Title                    = {Foundations of Signal Processing},
	Author                   = { Vetterli, M and Kovacevic, J and Goyal, V.K},
	Publisher                = {Cambridge University Press},
	Year                     = {2014}
}

@book{kolaczyck2009,
	title = {{S}tatistical {A}nalysis of {N}etwork {D}ata: {M}ethods and {M}odels},
	author = {E. D. Kolaczyk},
	publisher = {Springer, New York},
	year = {2009}
}
	
@inproceedings{segarra2016nodevariant, 
	title={Linear network operators using node-variant graph filters}, 
	author={S. Segarra and A. G. Marques and A. Ribeiro}, 
	booktitle={IEEE Trans. on Signal Processing}, 
	month = {Mar.},
	year={2016},
	address={Shanghai, China}, 
	pages={4850--4854} 
}
@ARTICLE{Chen15,
  author={S. {Chen} and R. {Varma} and A. {Sandryhaila} and J. {Kovačević}},
  journal={IEEE Transactions on Signal Processing}, 
  title={Discrete Signal Processing on Graphs: Sampling Theory}, 
  year={2015},
  volume={63},
  number={24},
  pages={6510-6523},}

@article{safavi2015nulling, 
	title={Revisiting Finite-Time Distributed Algorithms via Successive Nulling of Eigenvalues}, 
	author={S. Safavi and U. A. Khan}, 
	journal=ieeespl, 
	month={Jan.},
	year={2015}, 
	volume={22}, 
	number={1}, 
	pages={54--57}
}


@ARTICLE{Shuman2013GSP,
author={D. I. {Shuman} and S. K. {Narang} and P. {Frossard} and A. {Ortega} and P. {Vandergheynst}},
journal={IEEE Signal Processing Magazine},
title={The emerging field of signal processing on graphs: Extending high-dimensional data analysis to networks and other irregular domains},
year={2013},
volume={30},
number={3},
pages={83-98},
keywords={data analysis;data structures;feature extraction;graph theory;signal processing;open issues;high-dimensional graph data;information extraction;irregular graph data structures;classical frequency domain;graph spectral domains;computational harmonic analysis;spectral graph theoretic concepts;weighted graphs;high-dimensional data analysis;signal processing;Tutorials;Biological neural networks;Harmonic analysis;Spectral analysis;Frequency domain analysis},
doi={10.1109/MSP.2012.2235192},
ISSN={},
month={May},
}

@misc{grant2008cvx,
  title={{CVX}: Matlab software for disciplined convex programming},
  author={M. Grant, S. Boyd, and Y. Ye},
  year={2008}
}



@inproceedings{kibangou2012graph,
  title={Graph Laplacian based matrix design for finite-time distributed average consensus},
  author={Y. A. Kibangou},
  booktitle={American Control Conf.},
  month={Jun.},
  year={2012},
  address={Montreal,Canada},
  pages={1901--1906}
}

@ARTICLE{Coutino2019Advance,
author={M. {Coutino} and E. {Isufi} and G. {Leus}},
journal={IEEE Transactions on Signal Processing},
title={Advances in Distributed Graph Filtering},
year={2019},
volume={67},
number={9},
pages={2320-2333},
month={May.}
}

@article{Boyd2011ADMM,
author = {Boyd, Stephen and Parikh, Neal and Chu, Eric and Peleato, Borja and Eckstein, Jonathan},
year = {2011},
month = {01},
pages = {1-122},
title = {Distributed Optimization and Statistical Learning via the Alternating Direction Method of Multipliers},
volume = {3},
journal = {Foundations and Trends in Machine Learning}
}

@article{mateos2012drls,
title={Performance analysis of the consensus-based distributed LMS algorithm},
author={G. Mateos and I. D. Schizas and A. Ribeiro and G. B. Giannakis},
journal={EURASIP Journal on Advances in Signal Processing},
volume={},
number={},
pages={1-19},
month={Nov.},
year={2009},
}

@INPROCEEDINGS{Lorenzo19, 
author={P. {Di Lorenzo} and S. {Barbarossa} and S. {Sardellitti}}, booktitle={ICASSP 2019 - 2019 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)}, title={Distributed Signal Recovery Based on In-network Subspace Projections}, year={2019}, volume={}, number={}, pages={5242-5246},
}

@INPROCEEDINGS{LorenzoAsilomar,
author={P. {Di Lorenzo} and S. {Barbarossa} and S. {Sardellitti}}, booktitle={2019 53rd Asilomar Conference on Signals, Systems, and Computers}, title={Distributed Adaptive Learning of Graph Processes via In-Network Subspace Projections}, year={2019}, volume={}, number={}, pages={41-45},
}

@ARTICLE{Nassif20, 
author={R. {Nassif} and S. {Vlaski} and A. H. {Sayed}}, journal={IEEE Transactions on Signal Processing}, title={Adaptation and Learning Over Networks Under Subspace Constraints—Part I: Stability Analysis}, year={2020}, volume={68}, number={}, pages={1346-1360},
}

@ARTICLE{Shuman18, 
author={D. I. {Shuman} and P. {Vandergheynst} and D. {Kressner} and P. {Frossard}}, journal={IEEE Transactions on Signal and Information Processing over Networks}, title={Distributed Signal Processing via Chebyshev Polynomial Approximation}, year={2018}, volume={4}, number={4}, pages={736-751},
}

@ARTICLE{Shuman16, 
author={D. I. {Shuman} and B. {Ricaud} and P. {Vandergheynst}}, journal={Applied and Computational Harmonic Analysis}, title={Vertex-frequency analysis
on graphs}, year={2016}, volume={40}, number={2}, pages={260-291},
}

@INPROCEEDINGS{Ma16, 
author={J. {Ma} and W. {Huang} and S. {Segarra} and A. {Ribeiro}}, booktitle={2016 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)}, title={Diffusion filtering of graph signals and its use in recommendation systems}, year={2016}, volume={}, number={}, pages={4563-4567}
,}

@ARTICLE{Belkin6, 
author={M. {Belkin} and P. {Niyogi} and V. {Sindhwani}}, journal={The Journal of Machine Learning Research}, title={Manifold Regularization: A Geometric Framework for Learning from Labeled and Unlabeled Examples}, year={2006}, volume={7}, number={}, pages={2399–2434},
}

@ARTICLE{Segarra16reconstruct,
author={S. {Segarra} and A. G. {Marques} and G. {Leus} and A. {Ribeiro}}, journal={IEEE Transactions on Signal Processing}, title={Reconstruction of Graph Signals Through Percolation from Seeding Nodes}, year={2016}, volume={64}, number={16}, pages={4363-4378}
,}

@INPROCEEDINGS{Girault14, 
author={B. {Girault} and P. {Gonçalves} and E. {Fleury} and A. S. {Mor}}, booktitle={2014 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)}, title={Semi-supervised learning for graph to signal mapping: A graph signal wiener filter interpretation}, year={2014}, volume={}, number={}, pages={1115-1119}
,}

@INPROCEEDINGS{Isufi18, 
author={E. {Isufi} and P. {Di Lorenzo} and P. {Banelli} and G. {Leus}}, booktitle={2018 IEEE Statistical Signal Processing Workshop (SSP)}, title={Distributed Wiener-Based Reconstruction of Graph Signals}, year={2018}, volume={}, number={}, pages={21-25}
,}

@ARTICLE{oNUKI16, 
author={M. {Onuki} and S. {Ono} and M. {Yamagishi} and Y. {Tanaka}}, journal={IEEE Transactions on Signal and Information Processing over Networks}, title={Graph Signal Denoising via Trilateral Filter on Graph Spectral Domain}, year={2016}, volume={2}, number={2}, pages={137-148}
,}

@INPROCEEDINGS{Isufi17, 
author={E. {Isufi} and G. {Leus}}, booktitle={2017 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)}, title={Distributed sparsified graph filters for denoising and diffusion tasks}, year={2017}, volume={}, number={}, pages={5865-5869}
,}

@ARTICLE{Shuman18denoise, 
author={D. I. {Shuman} and P. {Vandergheynst} and D. {Kressner} and P. {Frossard}}, journal={IEEE Transactions on Signal and Information Processing over Networks}, title={Distributed Signal Processing via Chebyshev Polynomial Approximation}, year={2018}, volume={4}, number={4}, pages={736-751}
,}

@inproceedings{Defferrard16,
author = {Defferrard, Micha\"{e}l and Bresson, Xavier and Vandergheynst, Pierre},
title = {Convolutional Neural Networks on Graphs with Fast Localized Spectral Filtering},
year = {2016},
isbn = {9781510838819},
publisher = {Curran Associates Inc.},
address = {Red Hook, NY, USA},
booktitle = {Proceedings of the 30th International Conference on Neural Information Processing Systems},
pages = {3844–3852},
numpages = {9},
location = {Barcelona, Spain},
series = {NIPS’16}
}

@ARTICLE{Gama19,
author={F. {Gama} and A. G. {Marques} and G. {Leus} and A. {Ribeiro}}, journal={IEEE Transactions on Signal Processing}, title={Convolutional Neural Network Architectures for Signals Supported on Graphs}, year={2019}, volume={67}, number={4}, pages={1034-1049}
,}

@ARTICLE{Loukas15,
author={A. {Loukas} and A. {Simonetto} and G. {Leus}}, journal={IEEE Signal Processing Letters}, title={Distributed Autoregressive Moving Average Graph Filters}, year={2015}, volume={22}, number={11}, pages={1931-1935}
,}

@ARTICLE{Isufi17auto,
author={E. {Isufi} and A. {Loukas} and A. {Simonetto} and G. {Leus}}, journal={IEEE Transactions on Signal Processing}, title={Autoregressive Moving Average Graph Filtering}, year={2017}, volume={65}, number={2}, pages={274-288}
,}
@INPROCEEDINGS{Kibangou12,
author={A. Y. {Kibangou}}, booktitle={2012 American Control Conference (ACC)}, title={Graph Laplacian based matrix design for finite-time distributed average consensus}, year={2012}, volume={}, number={}, pages={1901-1906}
,}

@phdthesis{Girault15,
    title    = {Signal Processing on Graphs - Contributions to an
Emerging Field},
    school   = { École Normale Supérieure de Lyon},
    author   = {B. Girault},
    year     = {2015}
}

@ARTICLE{Sardellitti17,
  author={S. {Sardellitti} and S. {Barbarossa} and P. D. {Lorenzo}},
  journal={IEEE Journal of Selected Topics in Signal Processing}, 
  title={On the Graph Fourier Transform for Directed Graphs}, 
  year={2017},
  volume={11},
  number={6},
  pages={796-811},}
  
  @ARTICLE{Shafipour18,
  author={R. {Shafipour} and A. {Khodabakhsh} and G. {Mateos} and E. {Nikolova}},
  journal={IEEE Transactions on Signal Processing}, 
  title={A Directed Graph Fourier Transform With Spread Frequency Components}, 
  year={2019},
  volume={67},
  number={4},
  pages={946-960},}
  
  @ARTICLE{Predd06,
  author={J. B. {Predd} and S. B. {Kulkarni} and H. V. {Poor}},
  journal={IEEE Signal Processing Magazine}, 
  title={Distributed learning in wireless sensor networks}, 
  year={2006},
  volume={23},
  number={4},
  pages={56-69},}
  
  @ARTICLE{Datta06,
  author={S. {Datta} and K. {Bhaduri} and C. {Giannella} and R. {Wolff} and H. {Kargupta}},
  journal={IEEE Internet Computing}, 
  title={Distributed Data Mining in Peer-to-Peer Networks}, 
  year={2006},
  volume={10},
  number={4},
  pages={18-26},}
  
  @ARTICLE{Barbarossa5G,
  author={S. {Barbarossa} and S. {Sardellitti} and P. {Di Lorenzo}},
  journal={IEEE Signal Processing Magazine}, 
  title={Communicating While Computing: Distributed mobile cloud computing over 5G heterogeneous networks}, 
  year={2014},
  volume={31},
  number={6},
  pages={45-55},}
  
  @ARTICLE{Di-lorenzo20,
  author={P. {Di Lorenzo} and S. {Barbarossa} and S. {Sardellitti}},
  journal={IEEE Transactions on Signal Processing}, 
  title={Distributed Signal Processing and Optimization Based on In-Network Subspace Projections}, 
  year={2020},
  volume={68},
  number={},
  pages={2061-2076},
  }
  
  @BOOK{Sayedbook,
  author={A. H. {Sayed}},
  title={Adaptation, Learning, and Optimization over Networks}, 
	Publisher = { Foundations and Trends in Machine Learning},
  year={2014},
  volume={7},
  number={4-5},
  pages={311-801},}
  
  @book{Kay,
author = {Kay, Steven M.},
title = {Fundamentals of Statistical Signal Processing: Estimation Theory},
year = {1993},
isbn = {0133457117},
publisher = {Prentice-Hall, Inc.},
address = {USA}
}

@article{xiao2004average, 
	author={L. Xiao and S. Boyd},
		title={Fast linear iterations for distributed averaging}, 
	journal={Systems and Control Lettters}, 
	month={Sep.},
	year={2004}, 
	volume={53}, 
	number={1}, 
	pages={65--78}
}

	
	@ARTICLE{romero2017spacetime,
  author={D. {Romero} and V. N. {Ioannidis} and G. B. {Giannakis}},
  journal={IEEE Journal of Selected Topics in Signal Processing}, 
  title={Kernel-Based Reconstruction of Space-Time Functions on Dynamic Graphs}, 
  year={2017},
  volume={11},
  number={6},
  pages={856-869},}
	
	@ARTICLE{romero2017multikernel,
  author={D. {Romero} and M. {Ma} and G. B. {Giannakis}},
  journal={IEEE Transactions on Signal Processing}, 
  title={Kernel-Based Reconstruction of Graph Signals}, 
  year={2017},
  volume={65},
  number={3},
  pages={764-778},}
	
  
  @ARTICLE{nedic2018decentralized,
  author={A. {Nedić} and A. {Olshevsky} and M. G. {Rabbat}},
  journal={Proceedings of the IEEE}, 
  title={Network Topology and Communication-Computation Tradeoffs in Decentralized Optimization}, 
  year={2018},
  volume={106},
  number={5},
  pages={953-976},}
  
  @ARTICLE{Tay15,
  author={D. B. H. {Tay} and Z. {Lin}},
  journal={IEEE Signal Processing Letters}, 
  title={Design of Near Orthogonal Graph Filter Banks}, 
  year={2015},
  volume={22},
  number={6},
  pages={701-704},}
  
  @ARTICLE{Narang12,
  author={S. K. {Narang} and A. {Ortega}},
  journal={IEEE Transactions on Signal Processing}, 
  title={Perfect Reconstruction Two-Channel Wavelet Filter Banks for Graph Structured Data}, 
  year={2012},
  volume={60},
  number={6},
  pages={2786-2799},}
  
  @article{XU13,
author = {Xu, Yangyang and Yin, Wotao},
title = {A Block Coordinate Descent Method for Regularized Multiconvex Optimization with Applications to Nonnegative Tensor Factorization and Completion},
journal = {SIAM Journal on Imaging Sciences},
year = {2013},
volume = {6},
number = {3},
pages = {1758-1789}}

@ARTICLE{Isufi17random,
  author={E. {Isufi} and A. {Loukas} and A. {Simonetto} and G. {Leus}},
  journal={IEEE Transactions on Signal Processing}, 
  title={Filtering Random Graph Processes Over Random Time-Varying Graphs}, 
  year={2017},
  volume={65},
  number={16},
  pages={4406-4421},}
  
  @ARTICLE{Gama19control,
  author={F. {Gama} and E. {Isufi} and A. {Ribeiro} and G. {Leus}},
  journal={IEEE Transactions on Signal Processing}, 
  title={Controllability of Bandlimited Graph Processes Over Random Time Varying Graphs}, 
  year={2019},
  volume={67},
  number={24},
  pages={6440-6454},}
  
@ARTICLE{leila20,
  author={L. B. {Saad} and B. {Beferull-Lozano}},
  journal={IEEE Internet of Things Journal}, 
  title={Accurate Graph Filtering in Wireless Sensor Networks}, 
  year={2020},
  volume={},
  number={},
  pages={1-1},}
  
  @INPROCEEDINGS{Isufis17pars,
  author={E. {Isufi} and G. {Leus}},
  booktitle={2017 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)}, 
  title={Distributed sparsified graph filters for denoising and diffusion tasks}, 
  year={2017},
  volume={},
  number={},
  pages={5865-5869},}
  @ARTICLE{Wang,
  author={ {Sheng-De Wang} and  {Te-Son Kuo} and  {Chen-Fa Hsu}},
  journal={IEEE Transactions on Automatic Control}, 
  title={Trace bounds on the solution of the algebraic matrix Riccati and Lyapunov equation}, 
  year={1986},
  volume={31},
  number={7},
  pages={654-656},}
  
@inproceedings{scho10,
author = {Sch\"{o}lkopf, Bernhard and Herbrich, Ralf and Smola, Alex J.},
title = {A Generalized Representer Theorem},
year = {2001},
booktitle = {Proceedings of the 14th Annual Conference on Computational Learning Theory},
pages = {416–426}
}

@incollection{rahimi07,
title = {Random Features for Large-Scale Kernel Machines},
author = {Ali Rahimi and Recht, Benjamin},
booktitle = {Advances in Neural Information Processing Systems 20},
pages = {1177--1184},
year = {2008}
}
@ARTICLE{shen19,
  author={Y. {Shen} and G. {Leus} and G. B. {Giannakis}},
  journal={IEEE Transactions on Signal Processing}, 
  title={Online Graph-Adaptive Learning With Scalability and Privacy}, 
  year={2019},
  volume={67},
  number={9},
  pages={2471-2483},
  month={May.}
  }
  @article{Hazan16,
author = {Hazan, Elad},
title = {Introduction to Online Convex Optimization},
year = {2016},
volume = {2},
number = {3–4},
journal = {Found. Trends Optim.},
month = aug,
pages = {157–325}
}


  @book{Rencher,
author = {Alvin,C. Rencher and G. Bruce Schaalje},
title = {Linear Models in Statistics},
year = {2007},
publisher = {John Wiley $&$ Sons, Inc},
address = {USA}
}
@book{Vapnik,
  author = {Vapnik, Vladimir N.},
  title = {Statistical Learning Theory},
  year = {1998},
   publisher = {Wiley-Interscience}
}
@book{Scholkopf,
author = {Scholkopf, Bernhard and Smola, Alexander J.},
title = {Learning with Kernels: Support Vector Machines, Regularization, Optimization, and Beyond},
year = {2001},
publisher = {MIT Press}
}
@article{shen,
author = {Shen, Yanning and Chen, Tianyi and Giannakis, Georgios B.},
title = {Random Feature-Based Online Multi-Kernel Learning in Environments with Unknown Dynamics},
year = {2019},
issue_date = {January 2019},
publisher = {JMLR.org},
volume = {20},
number = {1},
journal = {J. Mach. Learn. Res.},
month = jan,
pages = {773–808}
}

@inproceedings{rudi,
author = {Rudi, Alessandro and Rosasco, Lorenzo},
title = {Generalization Properties of Learning with Random Features},
year = {2017},
publisher = {Curran Associates Inc.},
number = {11},
location = {Long Beach, California, USA},
series = {NIPS'17},
pages = {3218–3228}
}

@book{shalev,
  author={S. Shalev-Shwartz},
  title={Online Learning and Online Convex Optimization},
  year={2012},
publisher = {Now Foundations and Trends}
  }
  
  
@article{sang,
author = {Sang, Lifeng and Arora, Anish and Zhang, Hongwei},
title = {On Link Asymmetry and One-Way Estimation in Wireless Sensor Networks},
year = {2010},
volume = {6},
number = {2},
journal = {ACM Trans. Sen. Netw.},
month = mar,
pages = {12–25}
}

@article{zamola,
author = {Zamalloa, Marco and Krishnamachari, Bhaskar},
title = {An Analysis of Unreliability and Asymmetry in Low-Power Wireless Links},
year = {2007},
volume = {3},
number = {2},
journal = {ACM Trans. Sen. Netw.},
month = jun,
pages = {1–34}
}
